Improving Recurrent Neural Network Responsiveness to Acute Clinical Events

Predictive models in acute care settings must be able to immediately recognize precipitous changes in a patient's status when presented with data reflecting such changes. Recurrent neural networks (RNNs) have become common for training and deploying clinical decision support models. They frequently exhibit a delayed response to acute events. New information must propagate through the RNN's cell state memory before the total impact is reflected in the model's predictions. This work presents input data perseveration as a method of training and deploying an RNN model to make its predictions more responsive to newly acquired information: input data is replicated during training and deployment. Each replication of the data input impacts the cell state and output of the RNN, but only the output at the final replication is maintained and broadcast as the prediction for evaluation and deployment purposes. When presented with data reflecting acute events, a model trained and deployed with input perseveration responds with more pronounced immediate changes in predictions and maintains globally robust performance. Such a characteristic is crucial in predictive models for an intensive care unit.

==> bios.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

%%\begin{IEEEbiography}{David Ledbetter}
%Biography text here.
%\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{David Ledbetter} 
is a Senior Data Scientist at Children's Hospital Los Angeles. With an extensive experience in signal processing and deep learning, he now works closely with clinicians to bridge the gap between healthcare professionals and data scientists. He fosters communication and enables collaborations to solve real clinical problems that require significant cross-disciplinary expertise. He has a passion for training aspiring data scientists who are looking to break into healthcare to make a meaningful impact. Mr. Ledbetter holds a Bachelor of Science in Mathematics.
\end{IEEEbiographynophoto}


% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{Eugene Laksana} is Data Scientist at Children's Hospital Los Angeles. His interests lie in bridging the gap between clinical experts and data scientists by cultivating meaningful interdisciplinary collaborations. Mr. Laksana has Bachelor of Science in Computer Science from the University of Southern California.

\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Melissa Aczon} is a Senior Data Scientist at Children's Hospital Los Angeles. She works closely with CHLA’s ICU physicians to define clinically meaningful problems and develop algorithms to solve them using advanced computational techniques. Prior to joining CHLA, Dr. Aczon was a Principal Scientist at Arete Associates. She has a Bachelor of Science in Mathematics from Harvey Mudd College and a Ph.D. in Scientific Computing and Computational Mathematics from Stanford University.

\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Randall Wetzel} is a tenured Professor of Pediatrics and Anesthesiology at the University of Southern California and has served as an attending physician in pediatric critical care for over 40 years both at Johns Hopkins Hospital and at CHLA. Dr. Wetzel completed his undergraduate and medical degrees in the UK.  He then trained in pediatrics at Case Western’s Rainbow Babies and Children’s Hospital, Critical Care Medicine at Johns Hopkins Hospital and subsequently Anesthesiology at Hopkins.  He is board certified in Pediatrics, Pediatric Critical Care, Anesthesiology and Pediatric Anesthesiology. Additionally he received an MBA with a focus on information technology from Hopkins. Recently his research has involved data science applied to critical care medicine. He has served as the Director of Critical Care Medicine and as the Chairman of Anesthesiology Critical Care Medicine at CHLA. He has trained hundreds of residents and over 100 critical care fellows. He founded the Virtual Pediatric Intensive Care Unit focused on information technology and data science which has supported research for over 20 years and received federal, state and private funding.  He also founded Virtual Pediatric Systems which collects information of all admissions to over 160 pediatric ICUs in the United States. 
\end{IEEEbiographynophoto}


% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
